Physics potential for the measurement of sigma(Hvv)*BR(H->mu+mu-) at a 1.4 TeV CLIC collider

The potential for the measurement of the branching ratio of the Standard Model-like Higgs boson decay into a mu+mu- pair at 1.4 TeV CLIC is analysed. The study is performed using the fully simulated CLIC_ILD detector concept, taking into consideration all the relevant physics and the beam-induced backgrounds. Despite the very low branching ratio of the H->mu+mu- decay, we show that the product of the branching ratio times the Higgs production cross section can be measured with a statistical uncertainty of 38 percent, assuming an integrated luminosity of 1.5 ab^-1 collected in five years of the detector operation at the 1.4 TeV CLIC with unpolarised beams. With polarised beams (-80%, +30%), the statistical uncertainty is better than 25%.

==> include/coupling-unc-deriv.tex <==
The statistical uncertainty of the Higgs coupling to muons, \gHMuMu, can be derived if \gHMuMu is expressed in terms of directly measurable quantities. For example, starting from the proportionality,
\begin{equation}
\label{eq-sigmabr}
\sigmaBR \propto \frac{\gHWW^2 \times \gHMuMu^2}{\GH} \nonumber 
\end{equation}
and making the substitution,
\begin{equation}
\label{eq-coupling}
\frac{\gHWW^2}{\GH} = 
	\frac{\gHWW^4}{\GH} 
	\frac{\gHZZ^2}{\gHWW^2}
	\frac{1}{\gHZZ^2} 
\end{equation}
it becomes clear that one can write:
\begin{equation}
\label{eq-coupling-meas}
	\gHMuMu^2 \propto  
		\frac{\sigmaBR}{\sigma(\hnn)\times\BR(\PH \to \PW\PW^\ast)} 
		\times
		\frac{\sigma(\hnn) \times \BR(\PH \to \bb)}
			{\sigma(\PH\PZ) \times \BR(\PH \to \bb)} 
		\times
		\sigma(\PH\PZ) \times \BR(\PH \to \Plp\Plm)
\end{equation}

Here $\sigma(\PH\PZ) \times \BR(\PH \to \Plp\Plm)$ and $\sigma(\PH\PZ) \times \BR(\PH \to \bb)$ are measured at the 350 GeV CLIC stage and all other quantities at the 1.4 TeV stage. Adding up quadratically the relative uncertainties of the measured quantities in Eq. \ref{eq-coupling-meas} using values from Ref. \cite{CLIC_snowmass13} one gets,
\begin{equation}
\label{eq-coupling-unc}
	\frac{\delta\gHMuMu^2}{\gHMuMu^2} = 38.1\percent \oplus 1.1\percent \oplus 0.3\percent \oplus 1.0\percent \oplus 4.2\percent = 38.4\percent
\end{equation}
and finally,
\begin{equation}
\label{eq-coupling-unc}
	\frac{\delta\gHMuMu}{\gHMuMu} = 19.2\percent
\end{equation}

%Since the Higgs production cross-section in \wwfusion ($\sigma_{\hnn}(1.4\unit{TeV}) = 244 \unit{fb}$) can be determined at CLIC with a statistical precision better than 1\percent \cite{CLIC_snowmass13}, the branching ratio $\BR(\hmumu)$ and its statistical uncertainty can be extracted from Eq.\ \ref{eq-sigma}. Since the Higgs coupling to the \PW boson can be determined at CLIC with a precision $\delta\gHWW / \gHWW = 0.9\percent$, and the Higgs width with a precision of $\delta\GH / \GH = 0.22\percent$, the corresponding uncertainty of the Higgs coupling to muons, \gHMuMu, is estimated to be \couplingunc\percent. 


